DFT+U+V is equivalent to DFT+U with density-dependent hybridized projectors

Hubbard-corrected density-functional theory (DFT+$U$) is a popular tool for first-principles modeling of materials with localized $d$ or $f$ electrons, but its on-site corrections tend to over-localize charge and break covalent bonds. Inter-site $+V$ corrections were introduced to counter this and are now widely used, but a formal justification has been lacking. Here we show that -- to first order in $V/U$ -- inter-site corrections are exactly equivalent to on-site DFT+$U$ evaluated on a density-matrix-dependent redefinition of the Hubbard projectors, hybridized with those of neighboring sites, providing insight into the explicit mechanism by which $V$ affects covalency. If the projectors are held frozen, as is common practice, the equivalence partially breaks down. Beyond reinterpreting the formalism, these results sharpen the questions of how $V$ should be computed and what the Hubbard subspaces fundamentally are.

==> paperlabels.tex <==
\newlabel{hunds_j:start}{{\getpagewiselinenumber {35}}{1}{}{}{}}
\newlabel{hunds_j:end}{{\getpagewiselinenumber {39}}{1}{}{}{}}
\newlabel{eq:e_dftu}{{1}{1}{}{equation.0.1}{}}
\newlabel{eq:e_dftu@cref}{{[equation][1][]1}{[1][1][]1}{}{}{}}
\newlabel{gks:start}{{\getpagewiselinenumber {54}}{1}{}{}{}}
\newlabel{gks:end}{{\getpagewiselinenumber {56}}{1}{}{}{}}
\newlabel{degrade:start}{{\getpagewiselinenumber {61}}{1}{}{}{}}
\newlabel{degrade:end}{{\getpagewiselinenumber {66}}{1}{}{}{}}
\newlabel{point4:start}{{\getpagewiselinenumber {67}}{1}{}{}{}}
\newlabel{point4:end}{{\getpagewiselinenumber {84}}{2}{}{}{}}
\newlabel{linear_bath:start}{{\getpagewiselinenumber {84}}{2}{}{}{}}
\newlabel{linear_bath:end}{{\getpagewiselinenumber {94}}{2}{}{}{}}
\newlabel{eq:e_dftuv}{{3}{2}{}{equation.0.3}{}}
\newlabel{eq:e_dftuv@cref}{{[equation][3][]3}{[1][2][]2}{}{}{}}
\newlabel{mismatch_letter:start}{{\getpagewiselinenumber {140}}{2}{}{}{}}
\newlabel{mismatch_letter:end}{{\getpagewiselinenumber {146}}{2}{}{}{}}
\newlabel{eq:energy_identity}{{4}{2}{}{equation.0.4}{}}
\newlabel{eq:energy_identity@cref}{{[equation][4][]4}{[1][2][]2}{}{}{}}
\newlabel{fig:all_orbitals}{{1}{3}{The original $\phi ^{I\sigma }_m(\mathbf {r})$, block-diagonalizing $\varphi ^{I\sigma }_i(\mathbf {r})$, and doubly hybridized Hubbard projectors $\tilde {\varphi }^{I\sigma }_i(\mathbf {r}) = e^{2\hat S}\varphi ^{I\sigma }_i(\mathbf {r})$ of nickel in antiferromagnetic NiO for the minority spin channel. For simplicity, only one nickel atom (green) and its nearest-neighbor oxygen atoms (red) are shown. The left column (a--c) shows three of the five original Hubbard projectors, defined as orthogonalized pseudo-atomic orbitals oriented with the Cartesian axes. (The crystal structure happens to align with the Cartesian directions, but in general the orientation of these orbitals is arbitrary.) The second column (d--f) shows the block-diagonalizing projectors $\ket {\varphi ^{I\sigma }_i}$, \emph {i.e.}\ the eigenvectors of $\mathbf {n}^{II}$; unlike the original projectors, these are oriented with respect to the local chemical environment, with the octahedral crystal field and the exchange field of the antiferromagnetic ordering producing a $d_{x^2-y^2}$ orbital (d), a $d_{z^2}$ orbital (e), and a combination of the degenerate $t_{2g}$ orbitals (f). The third column (g--i) shows the doubly hybridized projectors; the first two weakly hybridize with the oxygen $2p$ orbitals. Panels j and k show the density difference between the first two hybridized and block-diagonalizing orbitals (orange regions positive, blue negative), revealing the increased antibonding character with the chemically relevant oxygens}{figure.1}{}}
\newlabel{fig:all_orbitals@cref}{{[figure][1][]1}{[1][2][]3}{}{}{}}
\newlabel{eq:explicit_s}{{5}{3}{}{equation.0.5}{}}
\newlabel{eq:explicit_s@cref}{{[equation][5][]5}{[1][2][]3}{}{}{}}
\newlabel{vu_note:start}{{\getpagewiselinenumber {191}}{3}{}{}{}}
\newlabel{vu_note:end}{{\getpagewiselinenumber {195}}{3}{}{}{}}
\newlabel{eq:delta_phi_uj0}{{6}{3}{}{equation.0.6}{}}
\newlabel{eq:delta_phi_uj0@cref}{{[equation][6][]6}{[1][3][]3}{}{}{}}
\newlabel{degenerate_pointer:start}{{\getpagewiselinenumber {224}}{3}{}{}{}}
\newlabel{degenerate_pointer:end}{{\getpagewiselinenumber {231}}{3}{}{}{}}
\newlabel{eq:chain_rule}{{7}{4}{}{equation.0.7}{}}
\newlabel{eq:chain_rule@cref}{{[equation][7][]7}{[1][4][]4}{}{}{}}
\newlabel{eq:vuv_rewritten}{{9}{4}{}{equation.0.9}{}}
\newlabel{eq:vuv_rewritten@cref}{{[equation][9][]9}{[1][4][]4}{}{}{}}
\newlabel{mismatch_compounds:start}{{\getpagewiselinenumber {323}}{4}{}{}{}}
\newlabel{mismatch_compounds:end}{{\getpagewiselinenumber {329}}{4}{}{}{}}
\newlabel{fig:potential_elements}{{2}{5}{The frozen-projector approximation reproduces the exact \gls {dftuv} potential in bulk antiferromagnetic nickel oxide to within a small residual (panels a--c), which can be almost entirely accounted for by a single analytic second-order term (panels d, e). Each panel shows the matrix elements of various potentials in the basis of block-diagonalizing orbitals $\{\varphi _i^{I\sigma }\}$ evaluated at the $\Gamma $-point. The matrices are subdivided by Hubbard site; one can clearly see the five $d$ orbitals of each Ni and the three $p$ orbitals of each O. (The unit cell contains four atoms: two Ni and two O.) Panel (a) shows the matrix elements of the full (\emph {i.e.}\ exact) \gls {dftuv} potential $\braopket {\varphi _i^{I\sigma }}{\hat {V}_U + \hat {V}_V}{\varphi _j^{J\sigma }}$. The on-site blocks of the potential are clearly diagonal in this basis (by design). Panel (b) shows the matrix elements of the approximate potential $\braopket {\varphi _i^{I\sigma }}{\hat {\tilde {V}}^{(0)\sigma }}{\varphi _j^{J\sigma }}$ (\cref {eq:vuv_rewritten}), which, as desired, closely replicate the full \gls {dftuv} potential: the differences between the two are shown in panel (c). Panel (d) shows the matrix elements of the potential $\braopket {\varphi _i^{I\sigma }}{\hat {\tilde {V}}^{(0)\sigma } + \hat {\tilde {V}}^{(2)\sigma }}{\varphi _j^{J\sigma }}$, where $\hat {\tilde {V}}^{(2)\sigma }$ is the higher-order correction (\cref {eq:v_u_hybrid_second_order}). This potential even more closely matches the full \gls {dftuv} potential, as shown by their difference in panel (e). Computational details can be found in \cref {sec:comp_details}}{figure.2}{}}
\newlabel{fig:potential_elements@cref}{{[figure][2][]2}{[1][4][]5}{}{}{}}
\newlabel{conclusion:start}{{\getpagewiselinenumber {348}}{5}{}{}{}}
\newlabel{conclusion:end}{{\getpagewiselinenumber {369}}{5}{}{}{}}
\newlabel{app:proof}{{}{5}{}{section*.6}{}}
\newlabel{app:proof@cref}{{}{[1][5][]5}{}{}{}}
\newlabel{eq:v_u_diagonalizing}{{10}{6}{}{equation.Alph0.10}{}}
\newlabel{eq:v_u_diagonalizing@cref}{{[equation][10][2147483647,0]10}{[1][6][]6}{}{}{}}
\newlabel{eq:v_v_diagonalizing}{{11}{6}{}{equation.Alph0.11}{}}
\newlabel{eq:v_v_diagonalizing@cref}{{[equation][11][2147483647,0]11}{[1][6][]6}{}{}{}}
\newlabel{eq:e_u_hat}{{12}{6}{}{equation.Alph0.12}{}}
\newlabel{eq:e_u_hat@cref}{{[equation][12][2147483647,0]12}{[1][6][]6}{}{}{}}
\newlabel{eq:n_ii_T}{{13}{6}{}{equation.Alph0.13}{}}
\newlabel{eq:n_ii_T@cref}{{[equation][13][2147483647,0]13}{[1][6][]6}{}{}{}}
\newlabel{eq:e_u_master}{{15}{6}{}{equation.Alph0.15}{}}
\newlabel{eq:e_u_master@cref}{{[equation][15][2147483647,0]15}{[1][6][]6}{}{}{}}
\newlabel{eq:energy_demand}{{16}{6}{}{equation.Alph0.16}{}}
\newlabel{eq:energy_demand@cref}{{[equation][16][2147483647,0]16}{[1][6][]6}{}{}{}}
\newlabel{eq:e_v_projector}{{17}{6}{}{equation.Alph0.17}{}}
\newlabel{eq:e_v_projector@cref}{{[equation][17][2147483647,0]17}{[1][6][]6}{}{}{}}
\newlabel{eq:v_v_projector}{{18}{6}{}{equation.Alph0.18}{}}
\newlabel{eq:v_v_projector@cref}{{[equation][18][2147483647,0]18}{[1][6][]6}{}{}{}}
\newlabel{eq:rho_vv}{{19}{6}{}{equation.Alph0.19}{}}
\newlabel{eq:rho_vv@cref}{{[equation][19][2147483647,0]19}{[1][6][]6}{}{}{}}
\newlabel{eq:s_defining}{{20}{6}{}{equation.Alph0.20}{}}
\newlabel{eq:s_defining@cref}{{[equation][20][2147483647,0]20}{[1][6][]6}{}{}{}}
\newlabel{eq:energy_alpha_eq_1}{{22}{6}{}{equation.Alph0.22}{}}
\newlabel{eq:energy_alpha_eq_1@cref}{{[equation][22][2147483647,0]22}{[1][6][]6}{}{}{}}
\newlabel{eq:potential_from_energy}{{23}{6}{}{equation.Alph0.23}{}}
\newlabel{eq:potential_from_energy@cref}{{[equation][23][2147483647,0]23}{[1][6][]6}{}{}{}}

